Describing and Predicting Online Items with Reshare Cascades via Dual Mixture Self-exciting Processes

It is well-known that online behavior is long-tailed, with most cascaded actions being short and a few being very long. A prominent drawback in generative models for online events is the inability to describe unpopular items well. This work addresses these shortcomings by proposing dual mixture self-exciting processes to jointly learn from groups of cascades. We first start from the observation that maximum likelihood estimates for content virality and influence decay are separable in a Hawkes process. Next, our proposed model, which leverages a Borel mixture model and a kernel mixture model, jointly models the unfolding of a heterogeneous set of cascades. When applied to cascades of the same online items, the model directly characterizes their spread dynamics and supplies interpretable quantities, such as content virality and content influence decay, as well as methods for predicting the final content popularities. On two retweet cascade datasets -- one relating to YouTube videos and the second relating to controversial news articles -- we show that our models capture the differences between online items at the granularity of items, publishers and categories. In particular, we are able to distinguish between far-right, conspiracy, controversial and reputable online news articles based on how they diffuse through social media, achieving an F1 score of 0.945. On holdout datasets, we show that the dual mixture model provides, for reshare diffusion cascades especially unpopular ones, better generalization performance and, for online items, accurate item popularity predictions.

==> sections/fig-true_teaser.tex <==
\begin{figure}[!tbp]
	\centering
	\includegraphics[width=0.47\textwidth]{images/cikm_experiment_size_prediction_teaser_selected}
	\vspace{-3mm}
	\caption{
		Prediction of final popularity with confidence intervals (mean $\pm$ the standard deviation) of an article shared on Twitter from \textit{breitbart.com}. The \textcolor{blue}{blue} line predicts the final popularity at varying times since the articles was published. Details about the generation of the plot is described in the online appendix~\citep{appendix}.
	}
	\label{fig:true_teaser}
	\vspace{-4mm}
\end{figure}

\TODO{MAR}{To massage into text.}
As an example, \cref{fig:true_teaser} depicts prediction of an article from an American far-right controversial news source, \textit{breitbart.com}, \revA{alleging financial benefits for Joe Biden in Ukraine.
The article kicked off an entire conspiracy theory, was subsequently reposted on numerous other news sites, and enjoyed considerable popularity on social media}.
Our models \revA{are able to} accurately predict its final popularity \revA{less then} $10$ hours after its publication, with \revA{narrowing} confidence intervals.

==> sections/intro.tex <==
\section{Introduction}
The prevalence of online social media platforms, such as Twitter, stimulates the dissemination of online items produced in other websites in forms including articles, photos and videos. In some cases, users share an online item to a social media platform where their followers can reshare, resulting in \textit{diffusion cascades} of reshares. The total amount of user attention the item attracts defines the item popularity. Being able to characterize and identify popular items has seen increasing interests~\citep{Zhao2015SEISMIC:Popularity,lukasik2016hawkes}. While it is intuitive to develop content-based modeling approaches~\citep{hu2016multimodal,wang2018retweet}, they require consistent updates and do not capture user interactions with online items. In this work, we aim to explicitly characterize online items based on how users interact with them through their diffusion cascades on social media.

Among the broad classes of models successfully applied to characterize the diffusions of online items~\citep{jin2013epidemiological,zhang2013social}, a class of point process based models, dubbed the Hawkes processes, has attracted growing attention~\citep{Zhao2015SEISMIC:Popularity,kong2019modeling}. 
Such processes learn from the temporal patterns of resharing events and from fine-grained features of online diffusions to produce explainable parameters to quantify the diffusion dynamics and predict popularity. 
Most modeling efforts are generally aimed towards popular diffusions, whereas unpopular ones are usually discarded --- \citet{Zhao2015SEISMIC:Popularity} only study cascades with at least $50$ retweets, and \citet{Mishra2016FeaturePrediction} threshold at $20$ retweets ---, the goal being to learn what makes a popular diffusion.

However, all online items experience varying temporal dynamics which lead to both ``successful'' and ``unsuccessful'' diffusions. In fact, it has been shown that luck is an important factor in online popularity~\citep{cheng2014can}, and that unpopular diffusions make up for a large portion of observed data. In order to quantify an online item based on its diverse diffusion dynamics, this paper aims to establish a procedure to leverage all diffusion cascades by jointly modeling them with two mixture models derived from Hawkes processes.


Specifically, in this work, we address three open questions concerning modeling diffusions of online items.


\citet{cheng2014can} have shown that the final popularities of retweet diffusions are unpredictable due to uncertainties contributed by various factors. 
Recent work from \citep{Rizoiu2017c} seconds this conclusion with distributions of final popularity where the same information has high probabilities of both remaining unknown or getting extremely popular. 
This suggests that learning from popular diffusions lead to modeling bias as multiple temporal dynamics tend to drive the diffusion of online items.
The first question remains open: \textbf{how do we model temporal dynamics of an online item taking all diffusion cascades into account properly and efficiently?} 
We answer the question through two steps. We first jointly model multiple diffusion sequences using a single Hawkes process by summing up their log-likelihood functions, and we show that this can be decoupled to two separate parts that model the content virality and the content influence decay (i.e., the decaying of influence from a reshare action), respectively.
Second, we relax the single Hawkes process assumption by designing a Borel mixture model accounting for the distribution of final event counts of Hawkes processes~\citep{daw2018queue}, namely the Borel distribution, and a kernel mixture model for capturing different influence decaying dynamics. The mixture models are fitted efficiently via the expectation-maximization (EM) algorithm~\citep{dempster1977maximum}.

The aforementioned joint modeling provides a way to describe online items with their temporal dynamics. Fitted parameters or derived quantities are commonly used for analyzing diffusions~\citep{Rizoiu2016ExpectingPopularity}, but have not been applied for quantifying content, leading to the question: \textbf{can we characterize online items with their temporal diffusions via the learnt mixture models?} From mixture model parameters fitted on related cascades of an online item, we build aggregated quantities and weight vectors. The quantities, $\hat{n}^*$ and $\hat{\theta}$, summarize item temporal dynamics in terms of content virality and content influence decay, whereas the weight vectors encode the dynamics as consistent feature representations. On two large-scale retweet cascade datasets about YouTube videos and news articles, we characterize online items at levels of categories, publishers and items with $\hat{n}^*$ and $\hat{\theta}$. For instance, we identify potential viral YouTube video publishers such as \textit{MBCentertainment} and \textit{VICTON} from observed publishers. We also examine clustering of item publishers and prediction of item categories based on the weight vectors. We find that clustering groups of publishers reflect content similarities where publishers of traditional news and controversial news form two separate communities. Within a major cluster, we locate groups of publishers that are known to produce conspiracy articles or far-right news. Moreover, the best performing classifier for identifying controversial news at an F1 score of $0.945$ by incorporating the proposed weight vectors.

Apart from applications on observed diffusions, another question follows --- \textbf{can we employ the fitted mixture models to improve final popularity predictions on future content?}
We leverage the information from observed online items of same publishers to model and quantify newly published items. On the two datasets, we demonstrate improved  generalization performance compared to~\citep{Mishra2016FeaturePrediction} and obtain the best performing final popularity predictor than a feature-based regressor and the state-of-the-art generative model~\citep{Zhao2015SEISMIC:Popularity}.
The Borel distribution also enables one to predict popularities with variances. As an example, \cref{fig:true_teaser} depicts prediction of an article from an American far-right controversial news source, \textit{breitbart.com}, where our models predict its final popularity accurately within the confidence intervals only $10$ hours after its publication.



In summary, the main contributions of this work are:
\begin{itemize}
    \item We refine the likelihood function of Hawkes processes to jointly model diffusions relating to same online items. We design procedures to uncover multiple temporal dynamics through a Borel mixture model and a kernel mixture model decoupled from Hawkes processes for fitting content virality and content influence decay, separately.
    \item We propose a set of tools for quantifying online items with aggregated quantities, $\hat{n}^*$ and $\hat{\theta}$, and weight vectors derived from fitted model parameters, together with methods for predicting item final popularities and variances.
    \item On two large retweet cascade datasets, we measure online items at levels of categories, publishers and items in terms of virality and influence decay. We explore the informativeness of weight vectors derived from fitted model parameters as features for predicting content categories. Eventually, we show that better generalization and popularity prediction performances are achieved on unseen online items compared to the state-of-the-art models.
\end{itemize}

\noindent {\bf Related work} Generative models are commonly employed for modeling temporal diffusions of online information. 
Such models are designed to predict final popularities \citep{Zhao2015SEISMIC:Popularity,bao2016modeling}, uncover hidden diffusion networks \citep{rodriguez2011uncovering} and detect rumors \citep{ma2016detecting}. 
The same tasks have also been approached using feature-driven models, which train machine learning algorithms that use temporal features --- statistical summaries of temporal patterns --- together with user features and content features~\citep{bakshy2011everyone,martin2016exploring}. 
However, to our knowledge, most of the prior work concentrate on popular cascades, and the complete temporal information of the unpopular diffusions is rarely considered.

Hawkes processes~\citep{hawkes1974cluster} are a class of self-exciting point processes --- past events excites future events happening --- widely applied in analyzing social media~\citep{Kobayashi2016TiDeH:Dynamics,farajtabar2015coevolve}, earthquake aftershocks \citep{ogata1988statistical}, crime rate~\citep{mohler2013modeling}, online advertising~\citep{parmar2017forecasting}, energy consumption~\citep{Li2016} and finance~\citep{bacry2015hawkes}.
Event-level and sequence-level clusterings of Hawkes processes have been discussed in~\citep{du2015dirichlet} and~\citep{yang2013mixture,xu2017dirichlet},
and particular attention has been given to applying combining Hawkes processes with deep learning techniques~\citep{cao2017deephawkes}.
The present work extends the prior literature in several ways.
We derive two separate mixture models from Hawkes processes, a Borel mixture model and a kernel mixture model, for modeling content virality and content influence decay. We apply the models to complete historical diffusion cascades for learning and quantifying temporal dynamics of online items.

\input{sections/fig-true_teaser}

